The quantum UV-IR map for line defects in $\mathfrak{gl}(3)$-type class $S$ theories

We consider the quantum UV-IR map for line defects in class $S$ theories of $\mathfrak{gl}(3)$-type. This map computes the protected spin character which counts framed BPS states with spin for the bulk-defect system. We give a geometric method of computing this map motivated by the physics of five-dimensional $\mathcal{N}=2$ supersymmetric Yang-Mills theory, and compute it explicitly in various examples. As a spin-off we propose a new way of computing a certain specialization of the HOMFLY polynomial for links in $\mathbb{R}^3$, as a sum over BPS webs attached to the link.

==> latexmkrc <==
@cus_dep_list = (@cus_dep_list, "svg pdf 0 svg2pdf");
sub svg2pdf {
   my $curdir = cwd();
   system("inkscape -D --export-pdf=\"$curdir/$_[0].pdf\" \"$curdir/$_[0].svg\""); }
$pdf_mode = 1;
$pdflatex = 'pdflatex %O -synctex=1 -interaction=nonstopmode %S';
do './gitinfo2.pm'

